Towards a Unified Quantum Protocol Framework: Classification, Implementation, and Use Cases

We present a framework for the unification and standardization of quantum network protocols, making their realization easier and expanding their use cases to a broader range of communities interested in quantum technologies. Our framework is available as an open-source repository, the Quantum Protocol Zoo. We follow a modular approach by identifying two key components: Functionality, which connects real-world applications; and Protocol, which is a set of instructions between two or many parties, at least one of which has a quantum device. Based on the different stages of the quantum internet and use-case in the commercialization of quantum communication, our framework classifies quantum cryptographic functionalities and the various protocol designs implementing these functionalities. Towards this classification, we introduce a novel concept of resource visualization for quantum protocols, which includes two interfaces: one to identify the building blocks for implementing a given protocol and another to identify accessible protocols when certain physical resources or functionalities are available. Such classification provides a hierarchy of quantum protocols based on their use-case and resource allocation. We have identified various valuable tools to improve its representation with a range of techniques, from abstract cryptography to graphical visualizations of the resource hierarchy in quantum networks. We elucidate the structure of the zoo and its primary features in this article to a broader class of quantum information scientists, physicists, computer science theorists and end-users. Since its introduction in 2018, the quantum protocol zoo has been a cornerstone in serving the quantum networks community in its ability to establish the use cases of emerging quantum internet networks. In that spirit we also provide some of the applications of our framework from different perspectives.

==> apx_list.tex <==
\subsection{List of protocols considered in this work} \label{App:ListofProt}

%\begin{center}
\begin{longtable}{l}
List of protocols\\
\hline
\endfirsthead
\multicolumn{1}{l}{Continued from previous page} \\
\hline

List of protocols \\

\hline
\endhead
\hline\multicolumn{1}{r}{Continued on next page} \\
\endfoot
\endlastfoot
\hline
GHZ-based Quantum Anonymous Transmission\\
Verifiable Quantum Anonymous Transmission\\
Uncloneable Encryption\\
Polynomial Code-based Quantum Authentication\\
Fast Quantum Byzantine Agreement\\
Quantum Bit Commitment\\
Quantum Strong Coin Flipping\\
Quantum Weak Coin Flipping\\
Gottesman and Chuang Quantum Digital Signature\\
Prepare and Measure Quantum Digital Signature\\
Measurement Device Independent Quantum Digital Signature (MDI-QDS)\\
Arbitrated Quantum Digital Signature\\
Blind Delegation of Quantum Digital Signature\\
Designated Verifiable Quantum Signature\\
Limited Delegation of Quantum Digital Signature\\
Quantum Proxy Signature\\
Multipartite Entanglement Verification\\
Quantum Fingerprinting\\
BB84 Quantum Key Distribution\\
Measurement Device Independent Quantum Key Distribution (MDI-QKD)\\
Device-Independent Quantum Key Distribution\\
Continuous-Variable Quantum Key Distribution (CV-QKD)\\
Quantum Leader Election\\
Quantum Cheque\\
Quantum Coin\\
Quantum Token\\
Wiesner Quantum Money\\
Quantum Oblivious Transfer\\
Quantum Secret Sharing using GHZ States\\
Verifiable Quantum Secret Sharing\\
Classical Fully Homomorphic Encryption for Quantum Circuits\\
Measurement-Only Universal Blind Quantum Computation\\
Prepare-and-Send Quantum Fully Homomorphic Encryption\\
Prepare-and-Send Universal Blind Quantum Computation\\
Pseudo-Secret Random Qubit Generator (PSQRG)\\
Prepare-and-Send Verifiable Universal Blind Quantum Computation\\
Measurement-Only Verifiable Universal Blind Quantum Computation\\
Prepare-and-Send Verifiable Quantum Fully Homomorphic Encryption\\
Secure Client-Server Classical Delegated Computation\\
Secure Multiparty Delegated Classical Computation\\
Secure Multiparty Delegated Quantum Computation\\
Secure Multiparty Delegated Classical Computation\\
State Teleporation\\
Gate Teleporation\\
Quantum Prover Interactive Proofs\\
Weak String Erasure\\
Self-verification \\
Cross-Platform verification of Intermediate Scale Quantum Devices\\
Cross Entropy Benchmarking\\
Cycle Benchmarking\\
Hamiltonian and Phase Estimation\\
Direct Fidelity Estimation\\
Estimate average Fidelity of quantum gates\\
Fidelity witnesses for fermionic quantum simulations\\
Fidelity witnesses for multi-partite entangled states\\
Fidelity witnesses for Gaussian bosonic\\
Fidelity witnesses for Ground States of local Hamiltonians\\
Probably Approximately Correctly Learning (PAC)\\
Robust online Hamiltonian learning\\
Compressed Quantum Process Tomography\\
Full Quantum Process Tomography with Linear inversion\\
Quantum Gate Set Tomography\\
Characterization of addressability by randomized benchmarking\\
Interleaved Randomised Benchmarking\\
Purity Benchmarking\\
Randomised Benchmarking with confidence\\
Robust characterization of leakage errors\\
Robust characterization of loss rates\\
Standard Randomised Benchmarking\\
Compressed Sensing Tomography\\
Full Quantum state tomography with Linear Inversion\\
Full Quantum state tomography with Maximum Likelihood Estimation\\
Full Quantum state tomography with Bayesian mean estimation (BME)\\
Full Quantum state tomography using confidence regions\\
Many-body quantum state tomography with neural networks\\
Matrix Product State tomography\\
Tensor Network Tomography\\
Quantum Volume Estimation\\
\end{longtable}
%\end{center}


==> sec_method.tex <==
\section{Methodology}
A great variety of quantum protocols have been introduced in the literature by different communities, including theoretical and experimental physicists, computer scientists and mathematicians.

After collecting protocols (see appendix \ref{App:ListofProt} for a list of selected functionalities that were entered in the current study), we categorised and presented them as follows. First, we determined their exact functionality as if they were one component of a modular application or system. Then, keeping this same approach, we extracted the relevant information about their security, efficiency and the minimum hardware requirements for their implementation if they have been provided by the authors. We also determined their network stage as introduced in \cite{wehner2018quantum} in order to have a view on the consistency of our approach for determining the requirements for such protocols to be implementable. The concepts behind the modular approach are presented in Sec.~\ref{sec:modular}. A categorization based on the following parameters~\cite{zoocategories} is available and a link to these pages is also tactfully placed on the concerned protocol/functionality page.
\begin{itemize}
   \item  (1) Fully Quantum Functionality (2) Quantum Enhanced Classical Functionality. These determine the utility of functionality in a pre-quantum and post-quantum world.
    \item Network Stages: Based on the various network stages identified in~\cite{wehner2018quantum}, we classify protocols based on whether they require (1) Prepare and Measure  (2) Entanglement, Quantum Memory (3) Few-qubit Quantum Computation (4) Fault-Tolerant Quantum Computation. Here protocols listed in $N$ require all components available at network Stage $\le N$
    \item (1) Two-Party Protocols (2) Multi-Party protocols. This categorization is essential since establishing secure multi-party protocols is a far more daunting task than a secure two-party protocol.
    \item (1) Universal Task, (2) Certification Protocols, (3) Building blocks.
\end{itemize}

We further categorized the protocols according to their functionality and provided a meaningful structure for describing both the functionalities and the protocols such that each community can find the appropriate information just by referring to the section corresponding to their interest without the need to read the whole paper. This resulted in the textual representation of the functionalities and the protocols which will be described in Sec.\ref{sec:TextRep}. 

To offer an even more compact view of each protocol's components and their relations with other protocols and components, we provide a visual representation: each protocol decomposition is inserted into a knowledge graph. This representation, detailed in Sec.~\ref{sec:KGRep}, allows for further semi-automated studies such as extracting the protocols that can be implemented given the availability of some physical resources, but also which functionalities could be useful enough to be turned into embedded services in future devices. 
